TeachBench: A Syllabus-Grounded Framework for Evaluating Teaching Ability in Large Language Models

Large language models (LLMs) show promise as teaching assistants, yet their teaching capability remains insufficiently evaluated. Existing benchmarks mainly focus on problem-solving or problem-level guidance, leaving knowledge-centered teaching underexplored. We propose a syllabus-grounded evaluation framework that measures LLM teaching capability via student performance improvement after multi-turn instruction. By restricting teacher agents to structured knowledge points and example problems, the framework avoids information leakage and enables reuse of existing benchmarks. We instantiate the framework on Gaokao data across multiple subjects. Experiments reveal substantial variation in teaching effectiveness across models and domains: some models perform well in mathematics, while teaching remains challenging in physics and chemistry. We also find that incorporating example problems does not necessarily improve teaching, as models often shift toward example-specific error correction. Overall, our results highlight teaching ability as a distinct and measurable dimension of LLM behavior.

==> section/teaching_cases.tex <==
{
    "role": "user",
    "content": "你是一位顶尖的数学导师。你的目标是帮助学生掌握解决问题所需的数学概念。\n\n重要规则：\n1. 使用提供的知识点和示例作为教学材料\n2. 专注于教授基础的数学概念和解题策略\n3. 一旦你认为学生掌握了所有的知识点，请你输出：**teach done**。你可以和学生进行确认，但是一定要由你来输出 **teach done**。\n\n你的教学方法：\n1. 使用提供的知识点和相关示例作为主要教学材料\n2. 将所需的知识点分解为易于理解的概念\n3. 可以创建简单的相关示例来说明每个概念（也可以参考提供的示例）\n4. 可以要求学生解决小练习，逐步培养所需技能\n5. 提供指导和建议，但让学生自己解决问题\n\n知识点及相关例题（例题用于教学参考）：\n请你依次讲解以下1个知识点：\n\n知识点1：函数的基本性质 > 函数概念与运算 > 函数的概念: 在某个变化过程中有两个变量 x, y , 如果对于 x 在某个实数集合 D 内的每一个确定的值, 按照某个对应法则 f , y 都有唯一确定的实数值与它对应, 那么 y 就是 x 的函数, 记作 y = f(x), x ∈ D。\n\n相关例题：\n\nLevel 1 例题：\n题目：（选择题）下列选项中，y是x的函数的是：\nA. y = x² + x + 1\nB. y² = x\nC. |y| = x\nD. y是小于x的最大整数\n答案：A\n解析：根据函数的定义，对于自变量x的每一个确定的值，y都有唯一确定的值与之对应。\nA. 对于任意一个x的值，y都有唯一确定的y = x² + x + 1的值与之对应，符合函数定义。\nB. 当x>0时，一个x的值对应两个y值（y = ±√x），例如x=4时，y=2或y=-2，不符合“唯一确定”的要求。\nC. 当x>0时，一个x的值对应两个y值（y = ±x），例如x=1时，y=1或y=-1，不符合“唯一确定”的要求。\nD. 选项描述不清晰，但根据常见的取整函数定义，例如y=floor(x-1)，则符合函数定义，但题目中的描述“y是小于x的最大整数”本身存在歧义，不如A选项明确。在标准的选择题中，A选项是最佳答案，因为它明确且普遍地表示了一个函数关系。根据函数定义的核心——“唯一对应性”进行判断，A是唯一正确的选项。 [7, 18]\n\nLevel 2 例题：\n题目：（填空题）已知函数 f(x) 的定义域为 [0, 2]，求函数 g(x) = f(x+1) + √(2-x) 的定义域。\n答案：[ -1, 1 ]\n解析：要求函数 g(x) 的定义域，需要同时满足构成 g(x) 的两部分 f(x+1) 和 √(2-x) 的定义域要求。\n1. 对于 f(x+1)，根据已知条件，f(x) 的定义域是 [0, 2]，这意味着函数的自变量（括号里的整体）必须在 [0, 2] 范围内。所以，0 ≤ x+1 ≤ 2。\n解这个不等式组：\n- 由 x+1 ≥ 0，得 x ≥ -1。\n- 由 x+1 ≤ 2，得 x ≤ 1。\n所以，f(x+1) 的定义域是 [-1, 1]。\n2. 对于 √(2-x)，根据根式有意义的条件，根号下的表达式必须非负。所以，2-x ≥ 0。\n解这个不等式，得 x ≤ 2。\n3. 函数 g(x) 的定义域是以上两个条件的交集。即 x 需要同时满足 x ∈ [-1, 1] 和 x ≤ 2。\n两个区间的交集为 [-1, 1]。\n因此，函数 g(x) 的定义域为 [-1, 1]。 [10, 13]\n\nLevel 3 例题：\n题目：（解答题）已知函数 f(x) 对任意实数 x, y 均有 f(x+y) = f(x) + f(y)，且当 x > 0 时，f(x) < 0。 \n(1) 求 f(0) 的值；\n(2) 判断 f(x) 的奇偶性并证明；\n(3) 如果 f(1) = -2，求 f(x) 在区间 [-3, 3] 上的最值。\n答案：(1) f(0) = 0\n(2) f(x) 是奇函数\n(3) 最大值为 f(-3) = 6，最小值为 f(3) = -6\n解析：(1) 在 f(x+y) = f(x) + f(y) 中，令 x = y = 0，可得 f(0+0) = f(0) + f(0)，即 f(0) = 2f(0)。解得 f(0) = 0。\n\n(2) f(x) 是奇函数。证明如下：\n在 f(x+y) = f(x) + f(y) 中，令 y = -x，可得 f(x-x) = f(x) + f(-x)，即 f(0) = f(x) + f(-x)。\n因为 f(0) = 0，所以 f(x) + f(-x) = 0，即 f(-x) = -f(x)。\n根据奇函数的定义，f(x) 是奇函数。\n\n(3) 首先，判断函数的单调性。\n设 x1 < x2，则 x2 - x1 > 0。根据题意，当 x > 0 时，f(x) < 0，所以 f(x2 - x1) < 0。\n因为 f(x) 是奇函数，并且 f(x+y) = f(x) + f(y)，所以 f(x2 - x1) = f(x2 + (-x1)) = f(x2) + f(-x1) = f(x2) - f(x1)。\n所以有 f(x2) - f(x1) < 0，即 f(x2) < f(x1)。\n这表明函数 f(x) 在其定义域 R 上是单调递减函数。\n\n因为 f(x) 是单调递减函数，所以它在闭区间 [-3, 3] 上的最值在区间的端点处取得。\n最大值为 f(-3)，最小值为 f(3)。\n\n利用 f(x+y) = f(x) + f(y) 和 f(1) = -2 计算 f(3) 和 f(-3)。\nf(2) = f(1+1) = f(1) + f(1) = -2 + (-2) = -4。\nf(3) = f(2+1) = f(2) + f(1) = -4 + (-2) = -6。\n由于 f(x) 是奇函数，f(-3) = -f(3) = -(-6) = 6。\n\n因此，f(x) 在区间 [-3, 3] 上的最大值为 f(-3) = 6，最小值为 f(3) = -6。 [20, 24]\n\n"
},
{
    "role": "assistant",
    "content": "今天我们聚焦一个核心知识点：函数的概念。目标是让你能\n- 准确判断“y是否是x的函数”；\n- 正确确定函数的定义域；\n- 在简单函数方程场景下，利用定义推理基本性质。\n\n一、什么是函数（核心定义）\n- 定义：在某个变化过程中有两个变量 x, y。如果对每一个 x（x 属于某个实数集合 D）按照某个对应法则 f，都有唯一确定的实数 y 与之对应，那么 y 就是 x 的函数，记作 y = f(x), x ∈ D。\n- 关键词：自变量 x（定义域 D）、对应法则 f、唯一性（每个 x 只能对应一个 y）。\n\n直观理解\n- “唯一性”是判断的关键：一个 x 不能对应两个不同的 y。\n- 用图像语言：竖直线检验。若任意一条竖直线与图像至多相交一次，则它是 y 关于 x 的函数。\n\n二、用例讲解（Level 1）\n题：下列选项中，y 是 x 的函数的是：\nA. y = x² + x + 1\nB. y² = x\nC. |y| = x\nD. y 是小于 x 的最大整数\n标准答案：A\n要点：\n- A：每个 x 给出唯一 y，符合函数定义。\n- B：当 x>0 时，一值 x 对应两个 y（±√x），不唯一。\n- C：当 x>0 时，一值 x 对应两个 y（±x），不唯一。\n- D：描述不够严谨。若写成 y = ⌊x⌋（不超过 x 的最大整数），则是函数；但原表述“y 是小于 x 的最大整数”有歧义。在标准选择题里，A 最明确无歧义。\n\n三、定义域的确定（Level 2 思路）\n例：已知 f(x) 定义域为 [0, 2]，求 g(x) = f(x+1) + √(2−x) 的定义域。\n步骤：\n1) f(x+1) 有意义 ⇔ x+1 ∈ [0,2] ⇔ x ∈ [−1,1]。\n2) √(2−x) 有意义 ⇔ 2−x ≥ 0 ⇔ x ≤ 2。\n3) g 的定义域 = 两者交集 = [−1,1]。\n\n通用技巧\n- 复合/平移：g(x) = f(ax+b)，则 ax+b 必须落在 f 的定义域里，解不等式得到 x 的范围。\n- 和/积/差/商：多个部分同时有定义，取交集；额外注意分母≠0。\n- 根式：被开方数 ≥ 0；对数：真数 > 0。\n\n四、函数方程的基本推理（Level 3）\n条件：f(x+y) = f(x) + f(y)，且当 x > 0 时，f(x) < 0。\n推理：\n1) 取 x=y=0：f(0)=2f(0) ⇒ f(0)=0。\n2) 取 y=−x：f(0)=f(x)+f(−x)，又 f(0)=0 ⇒ f(−x)=−f(x)，所以 f 是奇函数。\n3) 单调性：若 x1 < x2，则 x2−x1 > 0，题设给出 f(x2−x1) < 0。又 f(x2−x1)=f(x2)−f(x1)，故 f(x2)−f(x1)<0 ⇒ f 单调递减。\n4) 已知 f(1)=−2，则 f(2)=−4，f(3)=−6；由奇性 f(−3)=6。单调递减 ⇒ 在区间 [−3,3] 上最大值在左端点、最小值在右端点：max f(−3)=6，min f(3)=−6。\n\n五、常见误区\n- 把“一个 x 对应两个 y”的关系当函数（如 y²=x、|y|=x）。\n- 忽略定义域限制（根式、分母、对数等）。\n- 对描述不严谨的文字表述不加辨析（如“小于 x 的最大整数”与“取整函数”的区别）。\n\n六、小练习（请你独立完成并给出过程）\n1) 判断题（多选）：下列哪些是 y 关于 x 的函数？\n   a. y = |x|\n   b. y² = x + 1\n   c. |y| = x − 2\n   d. y = ⌊x⌋（不超过 x 的最大整数）\n   说明：选出所有是函数的选项，并简述理由。\n\n2) 定义域练习：\n   已知 f 的定义域为 (1, 5)。求 h(x) = f(2x − 1) + √(3 − x) + 1/(x − 2) 的定义域。\n   提示：分别写出每一部分的 x 条件，然后取交集并排除分母为 0 的点。\n\n3) 函数方程小题：\n   已知 f(x+y)=f(x)+f(y)，且当 x>0 时 f(x)>0；并给定 f(1)=3。\n   a) 求 f(0)。\n   b) 判断 f 的奇偶性并说明理由。\n   c) 证明 f 的单调性（递增或递减？）。\n   d) 计算 f(−2) 与 f(3)。\n   e) 求 f 在区间 [−2, 2] 上的最大值和最小值。\n\n你把三题的答案和思路发给我，我来逐一点评并补充。完成后我会确认你是否已经完全掌握本节内容。"
},
{
    "role": "user",
    "content": "好的，让我们一步一步来解答这些练习题。\n\n### 1) 判断题\n\n我们需要判断下列哪些是 \\( y \\) 关于 \\( x \\) 的函数：\n\na. \\( y = |x| \\)\n   - 这是一个绝对值函数，对于每一个 \\( x \\) 值，\\( y \\) 都有唯一确定的值。因此，这是一个函数。\n\nb. \\( y^2 = x + 1 \\)\n   - 当 \\( x > -1 \\) 时，\\( y \\) 可以有两个值，即 \\( y = \\sqrt{x+1} \\) 或 \\( y = -\\sqrt{x+1} \\)。因此，这不是一个函数。\n\nc. \\( |y| = x - 2 \\)\n   - 当 \\( x > 2 \\) 时，\\( y \\) 可以有两个值，即 \\( y = x - 2 \\) 或 \\( y = -(x - 2) \\)。因此，这不是一个函数。\n\nd. \\( y = \\lfloor x \\rfloor \\)\n   - 这是一个取整函数，对于每一个 \\( x \\) 值，\\( y \\) 都有唯一确定的值。因此，这是一个函数。\n\n**答案：a, d**\n\n### 2) 定义域练习\n\n已知 \\( f \\) 的定义域为 \\( (1, 5) \\)。求 \\( h(x) = f(2x - 1) + \\sqrt{3 - x} + \\frac{1}{x - 2} \\) 的定义域。\n\n- 对于 \\( f(2x - 1) \\)：要使 \\( f(2x - 1) \\) 有意义，\\( 2x - 1 \\) 必须在 \\( f \\) 的定义域内，即 \\( 1 < 2x - 1 < 5 \\)。解这个不等式得到 \\( 1 < x < 3 \\)。\n- 对于 \\( \\sqrt{3 - x} \\)：要使 \\( \\sqrt{3 - x} \\) 有意义，\\( 3 - x \\geq 0 \\)，即 \\( x \\leq 3 \\)。\n- 对于 \\( \\frac{1}{x - 2} \\)：要使 \\( \\frac{1}{x - 2} \\) 有意义，\\( x - 2 \\neq 0 \\)，即 \\( x \\neq 2 \\)。\n\n综合上述条件，我们得到 \\( 1 < x < 3 \\) 且 \\( x \\neq 2 \\)。因此，\\( h(x) \\) 的定义域为 \\( (1, 2) \\cup (2, 3) \\)。\n\n**答案：\\( (1, 2) \\cup (2, 3) \\)**\n\n### 3) 函数方程小题\n\n已知 \\( f(x + y) = f(x) + f(y) \\)，且当 \\( x > 0 \\) 时 \\( f(x) > 0 \\)；并给定 \\( f(1) = 3 \\)。\n\na) 求 \\( f(0) \\)。\n   - 取 \\( x = y = 0 \\)，则 \\( f(0 + 0) = f(0) + f(0) \\)，即 \\( f(0) = 2f(0) \\)。解得 \\( f(0) = 0 \\)。\n\nb) 判断 \\( f \\) 的奇偶性并说明理由。\n   - 取 \\( y = -x \\)，则 \\( f(x + (-x)) = f(x) + f(-x) \\)，即 \\( f(0) = f(x) + f(-x) \\)。由于 \\( f(0) = 0 \\)，则 \\( f(x) + f(-x) = 0 \\)，即 \\( f(-x) = -f(x) \\)。因此，\\( f \\) 是奇函数。\n\nc) 证明 \\( f \\) 的单调性（递增或递减？）。\n   - 设 \\( x_1 < x_2 \\)，则 \\( x_2 - x_1 > 0 \\)。根据题设，\\( f(x_2 - x_1) > 0 \\)。又 \\( f(x_2 - x_1) = f(x_2) - f(x_1) \\)，则 \\( f(x_2) - f(x_1) > 0 \\)，即 \\( f(x_2) > f(x_1) \\)。因此，\\( f \\) 是单调递增函数。\n\nd) 计算 \\( f(-2) \\) 与 \\( f(3) \\)。\n   - 由于 \\( f \\) 是奇函数，\\( f(-2) = -f(2) \\)。根据 \\( f(x + y) = f(x) + f(y) \\)，令 \\( x = 1 \\) 且 \\( y = 1 \\)，则 \\( f(2) = f(1) + f(1) = 3 + 3 = 6 \\)。因此，\\( f(-2) = -6 \\)。\n   - 同样地，\\( f(3) = f(2) + f(1) = 6 + 3 = 9 \\)。\n\ne) 求 \\( f \\) 在区间 \\([-2, 2]\\) 上的最大值和最小值。\n   - 由于 \\( f \\) 是单调递增函数，最小值出现在 \\( x = -2 \\)，最大值出现在 \\( x = 2 \\)。因此，最小值为 \\( f(-2) = -6 \\)，最大值为 \\( f(2) = 6 \\)。\n\n**答案：**\na) \\( f(0) = 0 \\)\nb) \\( f \\) 是奇函数\nc) \\( f \\) 是单调递增函数\nd) \\( f(-2) = -6 \\)，\\( f(3) = 9 \\)\ne) 最小值为 \\( -6 \\)，最大值为 \\( 6 \\)\n\n请检查我的解答是否正确，如果有任何问题或需要进一步解释的地方，请告诉我！"
},
{
    "role": "assistant",
    "content": "你的解答非常到位，三题都正确，理由清晰。\n\n针对每题给两点小补充，帮助你巩固要点：\n\n1) 判断题\n- c. |y| = x − 2 的细节：它的自然定义域是 x ≥ 2。虽然 x = 2 时只有 y = 0 一个值，但当 x > 2 时会出现两值 y = ±(x − 2)，从而不满足“每个 x 唯一对应 y”，因此整体不是函数。\n- d. 你写成 y = ⌊x⌋（不超过 x 的最大整数）是标准且无歧义的函数表述，这一点非常好。\n\n2) 定义域题\n- 你正确解出了 1 < 2x − 1 < 5 ⇒ 1 < x < 3，并注意到 √(3 − x) 给出 x ≤ 3（与前者相容）以及 x ≠ 2 的限制。\n- 交集和点剔除都处理正确，最终 (1, 2) ∪ (2, 3) 是标准答案。\n\n3) 函数方程题\n- a, b, c 的推理与结论都正确：f(0) = 0；f 为奇函数；由“x > 0 ⇒ f(x) > 0”可推出单调递增（与“单调递减”的对偶情况相呼应）。\n- d, e 数值一致且与单调性一致：f(−2) = −6，f(3) = 9；区间 [−2, 2] 上最小值 −6、最大值 6。\n- 额外一点见解（加深理解）：满足 f(x + y) = f(x) + f(y) 且单调的函数一定是线性的 f(x) = kx。由 f(1) = 3 得 k = 3，因此 f(x) = 3x。你算出的所有数值与此完全一致。\n\n从你的作答看，你已经准确掌握了：\n- 函数的“唯一对应性”判定原则；\n- 复合、根式、分母等情况下定义域的求法（取交集与点剔除）；\n- 简单函数方程下的基本性质推导（f(0)、奇偶性、单调性、端点取值）。\n\nteach done"
}
